The Midas Touch: Triggering the Capability of LLMs for RM-API Misuse Detection

In this paper, we propose an LLM-empowered RM-API misuse detection solution, ChatDetector, which fully automates LLMs for documentation understanding which helps RM-API constraints retrieval and RM-API misuse detection. To correctly retrieve the RM-API constraints, ChatDetector is inspired by the ReAct framework which is optimized based on Chain-of-Thought (CoT) to decompose the complex task into allocation APIs identification, RM-object (allocated/released by RM APIs) extraction and RM-APIs pairing (RM APIs usually exist in pairs). It first verifies the semantics of allocation APIs based on the retrieved RM sentences from API documentation through LLMs. Inspired by the LLMs' performance on various prompting methods,ChatDetector adopts a two-dimensional prompting approach for cross-validation. At the same time, an inconsistency-checking approach between the LLMs' output and the reasoning process is adopted for the allocation APIs confirmation with an off-the-shelf Natural Language Processing (NLP) tool. To accurately pair the RM-APIs, ChatDetector decomposes the task again and identifies the RM-object type first, with which it can then accurately pair the releasing APIs and further construct the RM-API constraints for misuse detection. With the diminished hallucinations, ChatDetector identifies 165 pairs of RM-APIs with a precision of 98.21% compared with the state-of-the-art API detectors. By employing a static detector CodeQL, we ethically report 115 security bugs on the applications integrating on six popular libraries to the developers, which may result in severe issues, such as Denial-of-Services (DoS) and memory corruption. Compared with the end-to-end benchmark method, the result shows that ChatDetector can retrieve at least 47% more RM sentences and 80.85% more RM-API constraints.

==> Sections/results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}
\label{sec:eval}

In this section, we assess the effectiveness of \toolname{} and its individual modules by comparing them with direct LLMs utilization and original human-written descriptions. Additionally, we also conduct a human study to evaluate the benefits of descriptions from \toolname{} in practice.


\subsection{Overall Effectiveness}
We first evaluate the effectiveness of \toolname{}, next we introduce the experiment setup and further analyze the results.
\subsubsection{Experiment Setup}

\textbf{Evaluation criteria.}

To accurately reflect the quality of descriptions in line with human understanding, it's crucial to select the right assessment metrics. Traditional evaluation metrics such as BLEU~\cite{papineni2002bleu}, ROUGE-L~\cite{Lin2004AutomaticEO} and METEOR~\cite{banerjee2005meteor} are not suitable for open-ended and knowledge-intensive tasks like security patch description. 

Specifically, these metrics use a ground-truth as a reference text and then compute the overlap between the generated text and the reference text to provide numerical scores. However, these metrics overlook critical aspects like accuracy and cannot effectively reflect the quality of the generated text.
For example, Figure~\ref{fig:desc-kzalloc-CVE-2019-19536} (b) and (c) show two generated descriptions for CVE-2019-19536's patch. Description 1 in Figure~\ref{fig:desc-kzalloc-CVE-2019-19536} (b) clearly explains the patch and its vulnerability. In contrast, description 2 in Figure~\ref{fig:desc-kzalloc-CVE-2019-19536} (c) wrongly describes vulnerability as a memory leak and incorrectly states the vulnerability triggering conditions. 
However, as revealed in Table~\ref{tab:compare-nlp-metrics}, when evaluating the two descriptions using the original developer-written patch descriptions as reference text, Description 2 scores better in BLEU and ROUGE-L than Description 1, despite the latter being more accurate. 
This shows that a higher traditional metrics score doesn't necessarily indicate superior description quality. 
Therefore, we perform manual evaluations. 

Specifically, we manually inspected whether the generated descriptions included three key elements: fixing operation, vulnerability cause, and security impacts. For each of these elements, we focus on both their presence and correctness. In other words, we check to see if the description describes this information and further determine if the description is correct. 


\begin{table}[ht]
\centering
\caption{Scores of descriptions using traditional NLP metrics}
\label{tab:compare-nlp-metrics}
\begin{tabular}{lccc}
\toprule
Description       & BLEU & ROUGE-L & METEOR \\
\midrule
Desc 1 (accurate) & 0.51 & 19.35 & \textbf{18.18} \\
Desc 2 (inaccurate) & \textbf{0.63} & \textbf{23.53} & 17.24 \\
\bottomrule
\end{tabular}
\end{table}

\noindent\textbf{Dataset construction.} We collect \todo{100} C security patches from the National Vulnerability Database (NVD) and PatchDB~\cite{wang2021patchdb}. The dataset covers prevalent vulnerability types like null-pointer-dereference, buffer overflow, resource leakage, and uninitialized use, which covers over 65\% of security patches~\cite{wang2023graphspd}. 


\noindent\textbf{Comparison method.} 
We evaluate \toolname{}'s effectiveness and its modules by comparing descriptions generated through the following methods:

\vspace{2pt}\noindent$\bullet$ \textit{LLM-basic:} The baseline, as described in Sec~\ref{llm-basic}, utilizes LLMs directly using code changes as code input and uses straightforward LLMs outputs.

\vspace{2pt}\noindent$\bullet$ \textit{\toolname{}--:} An enhancement of LLM-basic, \toolname{}-- incorporates the Prompt-Specific Construction module, which extracts relevant contexts to be provided to LLMs.

\vspace{2pt}\noindent$\bullet$ \textit{\toolname{}:} Augmenting \toolname{}--, this method introduces Code-Description Inconsistency Checking 


\noindent\textbf{LLMs setup.} We conduct evaluation under two representative LLMs from OpenAI: GPT-4~\cite{gpt-4} and GPT-3.5-turbo~\cite{gpt-3.5-turbo} (short for GPT-3.5).
They represent different capabilities of LLMs used for evaluating the generalizability of \toolname{}.

We access the models through the API provided by OpenAI. Specifically, we use the python library \texttt{openai} and request the models for results through the \texttt{ChatCompletion.create} function.
We set the temperature parameter to a mid-value of 0.5. We evaluate the three methods mentioned above with each model, e.g., LLM-basic$_{gpt3.5}$ means testing LLM-basic using GPT-3.5.


\subsubsection{Experiment Results}

Table~\ref{tab:overall-effectiveness} illustrates the comparison results of security patch description among various methods and models, focusing on four aspects: \textit{All}, \textit{Fixing operation}, \textit{Vulnerability cause}, and \textit{Security impacts}. The vertical axis presents the evaluated models, including LLM-basic, \toolname{}--, and \toolname{}, with GPT-3.5 and GPT-4 utilized. Additionally, we analyze human-written descriptions from the dataset, corresponding to the data shown in the human-written row. The \textit{All} column indicates the proportion of descriptions that accurately cover all three elements, while the remaining columns show the percentage of descriptions that correctly describe each specific element.



\begin{table}[thb]
\caption{Evaluation of patch descriptions across different methods and models}
\small
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{Mode}} 
& \textbf{All}
& \begin{tabular}[c]{@{}c@{}}\textbf{Fixing}\\\textbf{operation}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{Vuln}\\\textbf{cause}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}\textbf{Security}\\\textbf{impacts}\end{tabular} \\
\hline
Human-written             & 28\% & 54\% & 69\% & 73\% \\
\hline
LLM-basic$_{gpt3.5}$      & 16\% & 79\% & 30\% & 58\% \\
\toolname{}--$_{gpt3.5}$     & 31\% & 81\% & 36\% & 59\% \\
\textbf{\toolname{}$_{gpt3.5}$} & \textbf{37}\% & \textbf{86}\% & \textbf{44}\% & \textbf{67}\% \\
\hline
LLM-basic$_{gpt4}$        & 32\% & 91\% & 51\% & 60\% \\
\toolname{}--$_{gpt4}$       & 41\% & 98\% & 80\% & 79\% \\
\textbf{\toolname{}$_{gpt4}$} & \textbf{62}\% & \textbf{99}\% & \textbf{83}\% & \textbf{81}\% \\
\bottomrule
\end{tabular}
\vspace{3px}
\footnotesize
\\
Note: The percentages show patch descriptions' proportions that correctly describe each aspect. The percentage of All indicates the descriptions' percentage that correctly mentions all three elements.
\vspace{-8px}
\label{tab:overall-effectiveness}
\end{table}

\noindent\textbf{Overall effectiveness.}

The results reveal that \toolname{} improves security description generation across GPT-3.5 and GPT-4 models. Specifically, for the GPT-3.5 model, \toolname{} enhanced the percentage in the \textit{All} aspect by \todo{21\%} compared to LLM-basic. Under the GPT-4 model, the enhancement is more apparent, showing a \todo{30\%} increase. 
% This shows that improvements are not the same under different models.
These variances highlight that the effectiveness of \toolname{} varies with different models.
There is a correlation between model capabilities and \toolname{} effectiveness, and \toolname{} role is to stimulate the model's capabilities. Besides, the increases in the \textit{vulnerability causes} and \textit{security impacts} aspects are relatively higher than that for those in the \textit{fixing operations}. The main reason is that fixing operations is closely related to code changes, which is already provided by LLM-basic.

Besides, LLMs demonstrate distinct performances in describing different aspects of descriptions.
For instance, they perform better at describing the \textit{fixing operation}, achieving \todo{86\%} and \todo{99\%} with \toolname{}$_{gpt3.5}$ and \toolname{}$_{gpt4}$, respectively. In contrast, their performance for describing \textit{vulnerability cause} is not that good, with \todo{44\%} and \todo{83\%} for the respective models.  The possible reason is that describing \textit{fixing operation} is more direct, and requires more on summarizing code changes. Meanwhile, describing \textit{vulnerability cause} demands a deeper understanding of the context, thus it is more difficult for LLMs.


\noindent\textbf{Comparisons with human-written descriptions.} Notably, when compared with human-written descriptions, \toolname{}--$_{gpt4}$ stands out by achieving the highest scores across all four aspects: \textit{All}, \textit{Fixing operation}, \textit{Vulnerability cause}, and \textit{Security impacts}, scoring \todo{62\%}, \todo{99\%}, \todo{83\%}, and \todo{81\%} respectively. In contrast, human-written descriptions have lower scores, with \todo{28\%}, \todo{54\%}, and \todo{69\%}, \todo{73\%} respectively. One main reason is that while developers know their patches well, they sometimes miss important details in their descriptions. \toolname{}--$_{gpt4}$ provide detailed and accurate descriptions, showing its potential to improve the quality of security patch descriptions. 

Besides, descriptions generated by \toolname{} can inevitably contain some errors compared to human-written ones. It's important to note that developers are deeply familiar with their patches. And human-written descriptions, collected from the open-source community, have undergone reviews among developers, reducing the likelihood of errors. In contrast, \toolname{} might produce inaccuracies due to model limitations. Automatically correcting these inaccuracies is highly challenging. Nevertheless, such inaccuracies usually make up only a small part of the overall descriptions. With minor adjustments, developers can easily refine these descriptions for use.




\noindent\textbf{Effectiveness of patch-specific prompt construction.}
In particular, comparing \toolname{}-- with LLM-basic, we can see the patch-specific prompt construction module helps to increase the percentages of describing all three elements. For the \textit{All} aspect, it increases the percentage of by \todo{15\%} under the GPT-3.5 model, and \todo{9\%} under the GPT-4 model, respectively. \toolname{} improves input quality by incorporating patch context. In this way, LLMs not only enrich descriptions but also enhance their understanding of patches, thus producing more comprehensive descriptions.
Besides, \toolname{} displays more improvement in describing \textit{vulnerability causes} and \textit{security impacts}, compared to \textit{fixing operation}. LLM-basic provides code change information, which is directly related to \textit{fixing operation}, thus already enabling the LLMs to describe it directly. As contexts provide additional information about the vulnerability cause and the potential security impact, \toolname{}’s primary advancements are concentrated on the description of \textit{vulnerability cause} and \textit{security impact}.


\noindent\textbf{Effectiveness of code-description inconsistency checking.}
Comparing \toolname{} to \toolname{}--, we can see the effectiveness of the code-description inconsistency checking module. Under the GPT-3.5 model, the percentage of \textit{All} increased by \todo{6\%}, and under the GPT-4 model, it increased by \todo{21\%}. LLMs output is not only dependent on the quality of input data. It is also significantly influenced by LLMs' inherent capabilities. Therefore, with code-description inconsistency checking, \toolname{} can further improve the effectiveness using LLMs.


We analyze the cases where \toolname{} fails to correctly describe security-related details. These errors are not recognized by \toolname{} for three main reasons.
\ding{182} First, the unstructured nature of the text may hinder effective key-detail extraction thus preventing subsequent verification. 
For instance, \toolname{} overlooks the wrong fixing action \textit{``checks''} from the statement \textit{``The patches fix this by adding additional checks''} even though the code does not introduce new checks. 
\ding{183} Second, the vulnerability type and the corresponding fixing statement type are not one-to-one. Multiple vulnerability types may share the same statement type. For example, both memory leak and buffer overflow vulnerabilities might relate to call statements in patches. Thus, when a memory leak is misdescribed as a buffer overflow, \toolname{} cannot detect the inconsistency due to this overlap. \ding{184} Third, the description may contain errors about other types of information, such as the vulnerability trigger conditions, which are uncovered by \toolname{} currently. 


\subsection{Human Study}
To further evaluate if descriptions generated by \toolname{} can effectively help developers understand security patches, we conducted a human study. 

\noindent\textbf{Study setup.} We invited \todo{10} participants to evaluate patch descriptions, they have programming experience of \todo{5} to \todo{10} years. All of them are familiar with the C programming language and software security. 
We randomly selected \todo{10} security patches from the dataset. For each patch, we provided the original human-written description, LLM-basic$_{gpt4}$, and \toolname{}$_{gpt4}$, respectively. We asked participants to assess the usefulness, accuracy, and readability of the patch descriptions, with definitions of these aspects provided in Table~\ref{tab:human_study_aspects}. Particularly, usefulness and accuracy pertain to the content of the descriptions, well-written descriptions should be accurate and provide useful information for other developers to understand the fixing and the fixed vulnerability. Readability pertains to writing style, and well-written descriptions should be easy to read and understand. Participants rated these descriptions using a five-point Likert scale, where a score of 1 indicates strong disagreement and 5 denotes strong agreement.


\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Evaluation dimensions for human study}
\begin{tabular}{c|p{6cm}}
\toprule
\textbf{Dimension} & \textbf{Description} \\
\hline
Useful & The description is useful for understanding the patch and its vulnerability. \\
\hline
Accurate & The description accurately describes the vulnerability and patch-related information. \\
\hline
Readable & The description is easy to read and understand. \\
\bottomrule
\end{tabular}
\label{tab:human_study_aspects}
\end{table}



\begin{table}[h]
\centering
\caption{Comparison results in human study.}
\begin{tabular}{lllcc}
\toprule
Aspect   & Model          & Mean   & Median  \\
\midrule
\multirow{3}{*}{Useful}   & Human-written  & 3.99  & 4     \\
         & LLM-base       & 3.96  & 4    \\
         & \textbf{\toolname{}}    & \textbf{4.51}  & \textbf{5}      \\
\midrule
\multirow{3}{*}{Accurate}  & Human-written  & 4.2  & 4    \\
         & LLM-base       & 3.87  & 4      \\
         & \textbf{\toolname{}}    & \textbf{4.46}  & \textbf{5}      \\
\midrule
\multirow{3}{*}{Readable} & Human-written  & 4.11 & 4     \\
         & LLM-base       & 4.48   & 5      \\
         & \textbf{\toolname{}}    & \textbf{4.48}   & \textbf{5}     \\
\bottomrule
\end{tabular}
\label{tab:results-human-study}
\end{table}


% \todo{TODO:add results}
\noindent\textbf{Study results.} Each participant spent an average of \todo{33} minutes in total. 
% Each participant worked with \todo{10} security patches and spent an average of \todo{33} minutes in total. 
Table~\ref{tab:results-human-study} shows the results of human study across three dimensions: usefulness, accuracy, and readability. It includes the mean, median, and mode scores for each dimension.
The experimental results show that \toolname{} achieves the best results in all three dimensions: useful, accurate, and readable.
In particular, in terms of usefulness, \toolname{} achieved the highest mean score of \todo{4.51}, higher than both that of human-written and LLM-base. For accuracy, \toolname{} achieved the highest mean score of \todo{4.46}, whereas human-written and LLM-base descriptions had scores of \todo{4.2} and \todo{3.87}, respectively. A possible reason is that human-written descriptions fail to clearly describe the behaviors and vulnerabilities of patches but only give rough descriptions, while \toolname{} offers more specific and informative descriptions. Regarding readability, both \toolname{} and LLM-base achieved the highest mean score of \todo{4.48}, while human-written descriptions scored \todo{4.11}. A closer examination reveals that human-written descriptions occasionally contain spelling errors. Conversely, descriptions generated by LLMs are more fluent, relatively standardized, and thus also score better.

We also conducted the Wilcoxon Signed Rank test to assess the extent of developers’ agreement with the descriptions. Specifically, we evaluated whether descriptions from \toolname{} outperform human-written ones in terms of usefulness, accuracy, and reliability. The respective p-values for these categories are 1.54e-04, 4.75e-02, and 8.15e-04. Furthermore, we compared data from \toolname{} with those from LLM-basic in terms of usefulness, and accuracy, and the p-values are 6.03e-05 and 9.81e-05, respectively. Since all these p-values are below the threshold of 0.05, the differences are statistically significant.

We evaluate the effectiveness of prompt generation in \toolname, particularly the influence of patch code in the prompt. Given the inherent instability of models, simply evaluating result quality differences is insufficient to attribute enhancements to prompt generation. Hence, we adopt a targeted evaluation method. Specifically, we focus on information present in the context but missing in the original code changes, then inspect if LLMs' generated descriptions leveraged this contextual information for enhancement. For validation, 
we tested \todo{50} randomly selected patches, each of which generates 5 descriptions, and if at least one of the descriptions is improved, we consider the strategy is effective on that patch.

The experimental results show that the quality of \todo{xx\% of} the patches' descriptions is improved under GPT3.5, and \todo{70\% (35/50)} of the patches' descriptions are improved in GPT4. 
% Among these patches, we find that contexts help LLMs to understand patches more deeply. 
As contexts involve information such as the cause of the vulnerability, the potential security impact, or the triggering conditions, LLMs can not only add more details to the descriptions, but also improve the model's overall understanding of the patch, which in turn generates more accurate descriptions. 
For the remaining patches whose description quality does not improve, our analysis reveals the following reasons: first, \todo{eight} patches (e.g., replacing inappropriate functions or initialization operations) rely less on contextual information, and LLMs can describe patches using only code changes in conjunction with their inherent knowledge. Second, although some patches require context for understanding, LLMs fail to utilize this information due to its own limitations.
Overall, the prompt generation strategy is effective in improving output across models. Besides, this improvement is not always consistent due to the differences of models.}


==> Sections/results_new.tex <==
\section{Evaluation}
In this section, we evaluate the effectiveness of \toolname{}, comparing it against state-of-the-art patch description generation techniques and direct LLMs utilization. Additionally, we study the quality of real-world descriptions and explore the benefits of descriptions generated by \toolname{} for downstream tasks. 

% \subsection{Experiment Setup}


% We conduct evaluation under two representative LLMs from OpenAI: GPT-4~\cite{gpt-4} and GPT-3.5-turbo~\cite{gpt-3.5-turbo} (short for GPT-3.5).
% They represent different capabilities of LLMs used for evaluating the generalizability of \toolname{}.
 % \toolname{}.
% and cover different abilities.
% through the \texttt{ChatCompletion.create} function
% We evaluate the three methods mentioned above with each model, e.g., LLM-basic$_{gpt3.5}$ means testing LLM-basic using GPT-3.5.

\noindent\textbf{Environment.} Our experiments were conducted on Ubuntu 18.04 machine with 126 GB of RAM and 2 TB of storage. Computational tasks were accelerated using an NVIDIA GeForce RTX 3090, which has 24G of memory.

% \subsection{Overall Effectiveness}

\vspace{-6px}
\subsection{Compared with SOTA Techniques}
\label{compared-with-sota}
\ignore{
To evaluate the effectiveness of \toolname{} in generating security patch descriptions, we compared it with five patch description generation methods. Among these, four are from previous studies, and one directly uses LLMs as the baseline. A high-quality descriptions should accurately describe how patches fix vulnerabilities and underlying fixed vulnerabilities. To evaluate comprehensiveness and accuracy of descriptions, we utilize the powerful GPT-4 model~\cite{gpt-4}, 
GPT-4 demonstrates outstanding performance in text understanding. And the evaluation tasks did not involve complex reasoning or any code analysis. Additionally, to evaluate the generated descriptions quality more comprehensively, we also use three Natural Language Generation (NLG) metrics for evaluations.}

% To evaluate the effectiveness of \toolname{} in generating security patch descriptions, we compare it against state-of-the-art patch description generation techniques and the direct application of LLMs. 
The evaluation focuses on two key aspects: the comprehensiveness and accuracy of the descriptions. Furthermore, for a more thorough assessment of the description quality, we employ three Natural Language Generation (NLG) metrics for evaluations.
Next, we first introduce the experiment setup and detail the evaluations.

\noindent\textbf{Dataset Preparation.} In our experiments, we utilized the widely-used PatchDB~\cite{wang2021patchdb} security patches dataset. For manageability and to ensure cost-effectiveness, we collected 1,000 patches with high-quality descriptions, serving as reliable ground-truth references for evaluation. Specifically, we randomly sampled patches and confirmed whether their descriptions explained both patch behaviors and the reasons. This selection process was iterated until we collect 1,000 patches. Additionally, we preprocessed the descriptions to remove the additional information, which starts with special tags such as \texttt{Signed-off-by} and others. These tags, commonly used across various projects, typically convey additional metadata like authors and reviewers are unrelated directly to the patch content.

% appear at the end of descriptions and do not 
\ignore{
In our experiments, we utilized the widely-used PatchDB~\cite{wang2021patchdb} security patches dataset. To maintain manageability and cost-effectiveness, we randomly selected 1,000 security patches for our evaluation. To ensure the dataset's suitability for our evaluation, we preprocessed the descriptions to remove the additional information from descriptions, which starts with the special tags such as \texttt{Signed-off-by} and others. These tags, commonly used across various projects, typically convey additional metadata like authors and reviewers, appear at the end of descriptions and do not related directly to the patch content.}


\noindent\textbf{Compared techniques.}
\ignore{
Given the lack of research work dedicated to security patch description, we choose \todo{four} general-purpose patch description techniques for comparison. We downloaded the corresponding pre-trained models from the Hugging Face platform for evaluation, provided by JetBrains Research. 
These models were trained on the CommitChronicle~\cite{Eliseeva2023FromCM} dataset and fine-tuned for the commit message generation task.

\vspace{2pt}\noindent$\bullet$ \textit{CodeT5}~\cite{Wang2021CodeT5IU}: This is a pre-trained model designed for programming languages and natural language tasks. It is built based on the T5 model (Text-to-Text Transfer Transformer) and shows excellent performance in a variety of programming language tasks such as commit message generation.

\vspace{2pt}\noindent$\bullet$ \textit{CodeReviewer}~\cite{Li2022AutomatingCR}: this is a pre-trained model utilizing code change and code review data designed to support code review tasks. It can be fine-tuned for commit message generation.

\vspace{2pt}\noindent$\bullet$ \textit{RACE}~\cite{shi2022race}: This is a neural network based model which improves the quality of generation by retrieving similar commit messages. 
% RACE with CodeT5 as a backbone is state of the art in patch description generation.

\vspace{2pt}\noindent$\bullet$ \textit{RACE$_{history}$}~\cite{shi2022race,Eliseeva2023FromCM}: This is an enhanced version of RACE by adding commit message history as an additional context, this method performs best in generating commit messages at the time of writing.


\vspace{2pt}\noindent$\bullet$ \textit{LLM-basic:} \rewrite{As our baseline, LLM-basic employs a simple prompt template: \textit{``Write a commit message for the following patch code: {\{patch code\}}.''} This variant uses basic LLMs directly with straightforward instruction and the default patch code provided by git.}
}
Given the lack of research work dedicated to security patch description, we choose \todo{four} general-purpose patch description techniques for comparison: 

\vspace{2pt}\noindent$\bullet$ \textit{CodeT5}~\cite{Wang2021CodeT5IU}: A model designed for programming languages and natural language tasks. It shows excellent performance in various programming-related tasks, including commit message generation.

\vspace{2pt}\noindent$\bullet$ \textit{CodeReviewer}~\cite{Li2022AutomatingCR}: A pre-trained model utilizing code change and review data and designed for code review tasks. This model can also be adapted for generating commit messages.

\vspace{2pt}\noindent$\bullet$ \textit{RACE}~\cite{shi2022race}: A neural network-based model which improves generation quality by retrieving similar commit messages.
% to guide the generation.

\vspace{2pt}\noindent$\bullet$ \textit{RACE$_{history}$}~\cite{shi2022race,Eliseeva2023FromCM}: An advanced version of RACE that incorporates commit message history for additional context, this performs best in generating commit messages at the time of writing.

We downloaded the corresponding pre-trained models from the Hugging Face platform, provided by JetBrains Research. These models were trained on the CommitChronicle~\cite{Eliseeva2023FromCM} dataset for the commit message generation task.
Additionally, we established a baseline, \textit{LLM-basic}, which utilizes LLMs with direct instructions shown in Table~\ref{tbl:prompt-design} and the default patch code.

% code changes in patches. 



\ignore{
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{images/model_scores_per_metric_fixed_v2.pdf}
\caption{Prompt design for LLM-basic}
\label{fig:llm-baisc-prompt}
\end{figure}
}

\ignore{
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth]{images/performance_metrics_boxplot_separate_y.pdf}
\caption{Box plot of generation results}
\label{fig:boxplot}
\end{figure}
}

\ignore{
Table~\ref{tab:overall-study} presents average of METEOR, BLEURT and NUBIA on all the patch description generated by \toolname{} and compared techiniques. As shown by the table, \toolname{} outperforms all the compared techniques on all metrics significantly. 
For example, the improvements achieved \toolname{} 186.32\%, 30.40\%, and 57.47\%in METEOR, BLEURT and NUBIA, over the next highest score among the other models, respectively. Figure~\ref{fig:boxplot} further shows the distribution of METEOR, BLEURT, and NUBIA in a box plot.
The improvements achieved by \toolname{} (SecDescribler) are quite substantial across all evaluated metrics. The impressive improvements indicating \toolname{} generate descriptions that are more accurate (i.e., semantically closer to ground-truth), more fluent, more logical, and more grammatically accurate.
Specifically, in terms of METEOR, \toolname{} demonstrated an impressive improvement of approximately 186.32\% over the next highest score among the other techniques. For BLEURT, a metric assessing naturalness and fluency, \toolname{} showed a notable increase of 30.40\%. And in the NUBIA metric, evaluates the quality of text based on several aspects, including logic, relevance, and coherence, \toolname{} achieved an improvement of at least 57.47\%. 
These enhancements underscore the significant advancements that \toolname{} brings to the field of automated patch description generation.}


% \subsubsection{Evaluations of Completeness and accuracy}
\noindent\textbf{Evaluations of Comprehensiveness.} 
\ignore{
To evaluate the comprehensiveness of security patch descriptions, we focused on whether they include details on the \textit{what} (how the patches addresses vulnerabilities) and the \textit{why} (the vulnerabilities involved) aspects. To facilitate large-scale and automated evaluation, we employed GPT-4 for evaluations. GPT-4 is well-known for its outstanding performance in natural language understanding and the evaluation task focus solely on content classification without the need for complex reasoning or code analysis, ensures the reliability of results.}
To evaluate the comprehensiveness of security patch descriptions, we focused on whether they include details on \textit{what} the patches do and the reasons (\textit{why}) aspects. We utilized GPT-4 for large-scale, automated assessments due to its proficiency in natural language understanding, focusing on content classification without requiring complex reasoning or code analysis. 
% \rewrite{To ensure the reliability, we first aligned the assessment with human judgment. Initially, we manually annotated 100 patch descriptions to establish a benchmark. Subsequently, we refined the evaluation prompt, aiming for an accuracy threshold exceeding 90\%, to mirror human judgment closely.}
To guarantee the reliability, we aligned the assessment with human judgment by annotating 100 patch descriptions and refining the evaluation prompt to achieve over 90\% accuracy.
Specifically, we ask GPT-4 to classify descriptions into four types based on their content: both \textit{what} and \textit{why}, only \textit{what}, only \textit{why}, or neither. The used prompt is displayed in Table~\ref{tab:prompt_for_completeness_evaluation} in the Appendix.

\ignore{
Table~\ref{completeness-results} displays the overall comprehensiveness results for descriptions generated by various methods, including \toolname{} and other techniques. Each column represents the percentage of descriptions that cover both the \textit{what} and \textit{why} aspects (All), as well as those that include only the \textit{what} or \textit{why}, and neither (None).
The results shows that \toolname{} achieves a \todo{XX\%} rate in the All category, indicating that each patch description it generates successfully incorporates both an explanation of the patch behavior and the rationale.  In contrast, other methods including RACE, RACE$_{history}$, CodeReviewer, and CodeT5 present varied results, with at least \todo{XX\%} of the descriptions focusing solely on the \textit{what} aspect. They commonly struggle to explain the underlying vulnerabilities of security patches. Besides, these methods have about \todo{XX\%} of the generated descriptions lacking both the \textit{what} and the \textit{why}. Further analysis reveals that these descriptions are often have readability issues, such as providing only modified module paths without any natural language explanation. The overall results highlights the effectiveness of \toolname{} in generating comprehensive security patch descriptions.
}

Table~\ref{completeness-results} displays the comprehensiveness of descriptions generated by \toolname{} and comparative methods. Each column represents the percentage of descriptions that cover both the \textit{what} and \textit{why} aspects (All), as well as those that include only the \textit{what} or \textit{why}, and neither (None).
The results show that \toolname{} achieves a \todo{94\%} rate in the All category, indicating its ability to incorporate both patch behaviors and rationales within descriptions.
In comparison, methods like RACE, RACE$_{history}$, CodeReviewer, and CodeT5 have at least \todo{65\%} of the descriptions focus solely on the \textit{what} aspect, often omitting the critical \textit{why} aspect.
Besides, about \todo{30\%} of their descriptions also completely miss both aspects.
Further analysis reveals that these descriptions  often have readability issues, such as providing only modified code paths without any text explanation. Furthermore, LLM-basic also achieves a relatively high proportion, largely attributed to the well-designed prompt instruction and LLMs' capability to interpret it. However, for some patches, in the absence of context, LLM-basic tends to focus solely on code changes without providing reasons. In contrast, \toolname{} incorporates a broader context, enhancing LLM's ability to generate descriptions.
The results highlight \toolname{}'s effectiveness in generating comprehensive security patch descriptions.
% The results highlights the effectiveness of \toolname{} in generating comprehensive security patch descriptions.


\ignore{
\begin{table}[t]
\caption{Results of descriptions’ comprehensiveness across methods}
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Method} & \cellcolor{gray!25}\textbf{All} & \textbf{What} & \textbf{Why} & \textbf{None} \\ \hline
CodeT5 & \cellcolor{gray!25}25.96\% & 63.78\% & 0.10\% & 10.16\% \\ 
CodeReviewer & \cellcolor{gray!25}27.18\% & 62.58\% & 0.00\% & 10.24\% \\ 
RACE & \cellcolor{gray!25}24.30\% & 67.50\% & 0.00\% & 8.20\% \\ 
RACE$_{history}$ & \cellcolor{gray!25}26.08\% & 61.32\% & 0.13\% & 12.34\% \\ 
% message & 81.20\% & 16.59\% & 2.12\% & 0.10\% \\ \hline
LLM-basic & \cellcolor{gray!25}69.43\% & 30.57\% & 0.00\% & 0.00\% \\
\hline
\textbf{\toolname{}} & \cellcolor{gray!25}\textbf{100.00}\% & 0.00\% & 0.00\% & 0.00\% \\ \bottomrule
\end{tabular}
% \caption{Your table caption here.}
\label{completeness-results}
\end{table}}


\ignore{
\begin{table}[t]
\caption{\todo{Results of descriptions’ comprehensiveness across methods}}
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Method} & \cellcolor{gray!25}\textbf{All} & \textbf{What} & \textbf{Why} & \textbf{None} \\ \hline
RACE$_{history}$ & \cellcolor{gray!25}0.00\% & 6.00\% & 0.00\% & 94.00\% \\ 
RACE & \cellcolor{gray!25}0.00\% & 4.00\% & 0.00\% & 95.00\% \\ 
CodeReviewer & \cellcolor{gray!25}0.00\% & 5.00\% & 0.00\% & 95.00\% \\ 
CodeT5 & \cellcolor{gray!25}0.00\% & 3.00\% & 0.00\% & 97.00\% \\ 
LLM-basic & \cellcolor{gray!25}39.00\% & 59.00\% & 2.00\% & 0.00\% \\ 
\hline
% \textbf{\toolname{}} & \cellcolor{gray!25}\textbf{100.00}\% & 0.00\% & 0.00\% & 0.00\% \\ 
\toolname{} & \cellcolor{gray!25}45.27\% & 45.86\% & 5.33\% & 3.55\% \\
\bottomrule
\end{tabular}
% \caption{Your table caption here.}
\label{completeness-results}
\end{table}
}

\begin{table}[t]
\caption{Results of descriptions’ comprehensiveness across models}
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Model} & \cellcolor{gray!25}\textbf{All} & \textbf{What} & \textbf{Why} & \textbf{None} \\ \hline
RACE$_{history}$ & \cellcolor{gray!25}0\% & 69\% & 0\% & 31\% \\ 
% GPT-3.5 & \cellcolor{gray!25}96.00\% & 4.00\% & 0.00\% & 0.00\% \\ 
% GPT-3.5 Slicing & 
RACE & \cellcolor{gray!25}0\% & 70\% & 0\% & 30\% \\ 
CodeReviewer & \cellcolor{gray!25}0\% & 65\% & 0\% & 35\% \\ 
CodeT5 & \cellcolor{gray!25}0\% & 66\% & 0\% & 34\% \\
LLM-basic & \cellcolor{gray!25}87\% & 13\% & 0\% & 0\% \\ 
% LLM-basic & 
\hline
\toolname{} & \cellcolor{gray!25}94\% & 6\% & 0\% & 0\% \\
\bottomrule
\end{tabular}
\vspace{-8px}
\label{completeness-results}
\end{table}





\noindent\textbf{Evaluations of Semantic Accuracy.} 
\ignore{
To evaluate the semantic accuracy of the generated descriptions, we compared them with existing developer-written descriptions using semantic similarity as the metric. Specifically, we categorized the similarity into five distinct levels, ranging from 0 to 4, each defined by detailed scoring criteria presented in Table~\ref{scoring-criteria}. Then we utilized GPT-4 to assess semantic similarity between the given ground truth (developer-written descriptions) and the generated descriptions, assigning scores accordingly. The prompt is displayed Table~\ref{tab:semantic_similarity_prompt} in the Appendix.}
\ignore{
To evaluate the semantic accuracy of descriptions generated by \toolname{}, we used semantic similarity metrics to compare them against developer-written descriptions. Specifically, we defined five levels of similarity (0 to 4), with specific criteria for each level outlined in Table~\ref{scoring-criteria}. Using GPT-4, we evaluated the similarity of \toolname{}'s descriptions to these original descriptions, assigning scores accordingly. The evaluation prompt is displayed Table~\ref{tab:semantic_similarity_prompt} in the Appendix.
}
Given the challenge in precisely evaluating semantic accuracy, we followed common practices by measuring the semantic similarity to the ground truth. A higher degree of semantic similarity indicates that the generated descriptions more closely align with developers' intentions, indicating greater accuracy. Specifically, we defined five levels of similarity (0 to 4), with specific criteria for each level outlined in Table~\ref{scoring-criteria}. For the evaluation, we utilized GPT-4, initially refining the prompt to ensure the assessment's alignment with human evaluations. GPT-4 then scored the similarity of \toolname{}-generated descriptions to the developer-written ones. The evaluation prompt is displayed Table~\ref{tab:semantic_similarity_prompt} in the Appendix.


\begin{table}[h]
\centering
\small
\caption{Scoring criteria for semantic similarity}
\renewcommand{\arraystretch}{1.2}
\label{tab:scoring_criteria}
\begin{tabular}{c|p{0.85\columnwidth}}
\toprule
\textbf{Score} & \textbf{Description} \\
\midrule
0 & Unrelated: No semantic or lexical overlap. \\
1 & Slightly related: Some shared tokens, but semantically irrelevant. \\
2 & Partially similar: Some semantic overlap. \\
3 & Highly similar: Closely aligned semantically, but not identical. \\
4 & Identical: Semantically identical. \\
\bottomrule
\end{tabular}
\vspace{-8px}
\label{scoring-criteria}
\end{table}

Table~\ref{semantic_acc} presents the averaged semantic similarity scores for each method, along with the distribution across five levels (0 to 4). The results show that \toolname{} outperforms other methods with an average score of \todo{2.65}, indicating a closer alignment with developer-written descriptions.
% thus achieving a higher accuracy.
Specifically, \todo{71\%} of \toolname{}' generated descriptions exhibit high semantic similarity with the ground truth. Conversely, the total percentage for the lowest relevance scores (0, 1) is less than \todo{4\%}, indicating minimal occurrences of low-quality descriptions.
In comparison, existing methods such as CodeT5, CodeReviewer, RACE, and RACE$_{history}$ demonstrate nearly \todo{50\%} of their descriptions scoring a 2, indicating only partial similarity with the ground truth. While LLM-basic performs better than existing methods, it still falls short of \toolname{}'s effectiveness.
On the one hand, \toolname{} incorporates patch context into prompts. By doing so, LLMs gain a better understanding of the patches. Moreover, LLM generated-description is not only dependent on the quality of input data. It is also influenced by LLMs' inherent capabilities. \toolname{} identifies inaccuracies and filters them out, such as the inaccuracies shown in Figure~\ref{fig:desc-kzalloc-CVE-2019-19536} , thus further improving the descriptions' accuracy.
% These results highlight \toolname{}'s capability in generating semantically accurate descriptions.

\begin{table}[t]
\centering
\small
\caption{Results of descriptions’ semantic accuracy across methods}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
\textbf{Method} & \cellcolor{gray!25}\textbf{Avg} & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} \\ \hline
CodeT5 & \cellcolor{gray!25} 2.15 & 5\% & 11\% & 48\% & 36\% & 0\% \\
CodeReviewer & \cellcolor{gray!25}2.23 & 3\% & 9\% & 50\% & 38\% & 0\% \\
RACE & \cellcolor{gray!25}2.33 & 2\% & 6\% & 49\% & 43\% & 0\% \\
RACE$_{history}$ &\cellcolor{gray!25}2.27 & 2\% & 10\% & 47\% & 41\% & 0\% \\
% LLM-basic & \cellcolor{gray!25}2.57 & 1.60\% & 2.79\% & 32.31\% & 63.30\% & 0.00\% \\ \hline
LLM-basic & \cellcolor{gray!25}2.55 & 4\% & 3\% & 27\% & 66\% & 0\% \\
\hline
\textbf{\toolname{}} & \cellcolor{gray!25}2.65 & 2\% & 2\% & 25\% & 71\% & 0\% \\ 
\bottomrule
\end{tabular}
\label{semantic_acc}
\end{table}



% \subsubsection{Evaluations of automatic metrics.}

% \noindent\textbf{Evaluation criteria.}
\ignore{
Referring to previous work, we use developer-written descriptions as the ground-truth and score them by comparing the similarity between the generated text and the reference text. First, let us outline the chosen metrics and the rationale behind them. Our task is generative, not translational, and is an open-ended problem. Traditional metrics such as BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin2004rouge} are assessed only by simple word overlap and may not be highly relevant to human judgment. Traditional BLEU and ROUGE tend to be inaccurate because they focus on surface-level similarities; typically, there are many sentences that convey exactly the same meaning. In contrast, overlap-based metrics that rely only on lexical matching can only identify sentences that are only superficially similar in form, even if they do not accurately capture the true meaning of the sentence. BLEURT is more accurate than BLEU.
In order to gain a deeper understanding of the semantic quality of the text, we have selected the following three evaluation metrics, which show better performance for NLG (natural langugage generation) task evaluation:
}
\ignore{
To evaluate the quality of the security patch descriptions generated, we reference developer-written descriptions as ground truth and mainly evaluate the generated description's similarity to this ground truth. As the generative and open-ended nature of security patch description, we don't choose traditional metrics like BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin2004rouge}, which mainly focus on surface-level word overlaps and may not align well with human judgment in NLG (Natural Language Generation) evaluation. To effectively the quality of the generated descriptions, we employ the following metrics. By using these three metrics, we get a more comprehensive understanding of the generated text's quality.}

\ignore{
As the generative and open-ended nature of security patch description, we don't choose traditional metrics like BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin2004rouge}, which mainly focus on surface-level word overlaps and may not align well with human judgment in NLG (Natural Language Generation) tasks. Instead, we employed advanced NLG metrics such as METEOR, BLEURT, and NUBIA, using developer-written descriptions as the ground truth.
These metrics offer a deeper insight into the quality of the generated content. The following section details these metrics and the results:}
\noindent\textbf{Evaluations of automatic NLG metrics.}
To gain deeper insights into the quality of generated descriptions.
We further include three NLG metrics: METEOR, BLEURT, and NUBIA for evaluations. 
Unlike traditional metrics such as BLEU and ROUGE, which focus primarily on surface-level word overlaps, these selected metrics offer a more accurate assessment aligned with human judgment in Natural Language Generation tasks. For evaluated metrics, we take the original developer-written descriptions as ground truth. The following section details these metrics and the results:


\vspace{2pt}\noindent$\bullet$ \textit{METEOR} (Evaluation of Translation with Explicit Ordering)~\cite{banerjee2005meteor}: Beyond simple word-level precision and recall, METEOR also incorporates synonymy and stemming, better assessing semantic similarity between the generated and reference descriptions.

% This metric not only evaluates word-level precision and recall, but also takes into account the use of synonyms, and employs stemming and synonym matching techniques to more accurately capture the semantic similarity between the generated text and the reference text.

% \vspace{2pt}\noindent$\bullet$ \textbf{BLEURT} (Bilingual Evaluation Understudy with Representations from Transformers)~\cite{Sellam2020BLEURTLR}: This is a trained metric that evaluates the fluency of the candidate text and the extent to which it conveys the meaning of the reference text. It is pre-trained on a large amount of manually rated data, the It is able to capture the nuances and linguistic diversity of human raters.
% BLEURT is more accurate than BLEU.

\vspace{2pt}\noindent$\bullet$ \textit{BLEURT} (Bilingual Evaluation Understudy with Representations from Transformers)~\cite{Sellam2020BLEURTLR}: As a learned metric, BLEURT leveraging a large corpus of manually rated data to align closely with human judgment, which is shown to be more accurate than BLEU. It evaluates the fluency of the generated descriptions and the extent to which it conveys the meaning of the reference descriptions.

\vspace{2pt}\noindent$\bullet$ \textit{NUBIA} (Neural Based Interchangeability Assessor)~\cite{kane2020nubia}: Integrating multiple advanced language models such as RoBERTa STS, RoBERTa MNLI and GPT-2, NUBIA offers a comprehensive assessment across various fluency and semantic dimensions, outperforming traditional metrics like BLEU and ROUGE in NLG evaluation.

% By using these three indicators, we are able to comprehensively assess the fluency and semantic accuracy of the generated text, so as to understand and evaluate the quality of the generated text in a more comprehensive way.


% This way, we can better understand and score the quality of the generated descriptions. 

\begin{table}[ht]
\vspace{5px}
% \caption{Overall patch description generation results}
\caption{Results of the three metrics across methods}
\centering
\small
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccc}
\toprule
\textbf{Method} & \textbf{METEOR~\cite{banerjee2005meteor}} & \textbf{BLEURT}~\cite{Sellam2020BLEURTLR} & \textbf{NUBIA}~\cite{kane2020nubia} \\
\toprule
CodeT5         & 5.52      & 30.98   & 34.37          \\
CodeReviewer   & 5.61      & 31.16   & 34.72          \\
RACE           & 5.93   & 31.94      & 34.28         \\

RACE$_{history}$  & 5.43    & 31.89    & 34.99          \\
% LLM-basic & 11.62 & 38.09 & 44.03 \\
LLM-basic & 16.23 & 39.09 & 54.10 \\
\hline
% \textbf{\toolname{}}  & \textbf{16.99}    & \textbf{41.65}           & \textbf{55.10}  \\   
\textbf{\toolname{}}  & \textbf{17.11}    & \textbf{41.64}           & \textbf{56.11}  \\   
\bottomrule  
\end{tabular}
\vspace{-8px}
\label{tab:overall-study}
\end{table}

% gpt3.5 {'BLEU': 1.434, 'ROUGE-L': 19.166, 'METEOR': 16.989, 'BLEURT': 41.651, 'NUBIA': 55.1}
% gpt3.5_slicing {'BLEU': 1.443, 'ROUGE-L': 18.712, 'METEOR': 17.113, 'BLEURT': 41.643, 'NUBIA': 56.105}

% Figure~\ref{fig:boxplot} further illustrates the distribution of these metrics. 
\ignore{
In Table~\ref{tab:overall-study}, we present the average scores for METEOR, BLEURT, and NUBIA for all patch descriptions generated by \toolname{} and the compared techniques. 
\toolname{} demonstrates a notable enhancement over competing techniques, with improvements of \todo{186.32\%}, \todo{30.40\%}, and \todo{57.47\%} in METEOR, BLEURT, and NUBIA, respectively, when compared to the second-highest scores achieved by the other methods. These metrics, assessing semantic accuracy(through the evaluation of semantic similarity with the ground-truth), fluency, and logical coherence, indicate that \toolname{}'s generated descriptions are significantly more accurate, fluent, and logically consistent. Specifically, \toolname{} shows an impressive \todo{186.32\%} improvement in METEOR, a metric for semantic accuracy, a \todo{30.40\%} increase in BLEURT for semantic accuracy and fluency, and a \todo{57.47\%} improvement in NUBIA, which evaluates the quality of descriptions across various dimensions, including  logic, relevance, and coherence. These substantial enhancements demonstrate the capabilities of \toolname{} in security patch description generation.}

In Table~\ref{tab:overall-study}, we present the performance of \toolname{} against other methods using the METEOR, BLEURT, and NUBIA metrics for all generated patch descriptions. \toolname{} outperforms the existing methods with significant improvements: \todo{188\%} in METEOR, which evaluates semantic accuracy; \todo{30\%} in BLEURT, assessing both semantic accuracy and fluency; and \todo{60\%} in NUBIA, which considers logic, relevance, and coherence in the descriptions. These results demonstrate \toolname{}'s capabilities to generate security patch descriptions that are not only semantically accurate but also fluent and logically coherent.
% METEOR: (17.11-5.93)/5.93
% BLEURT: (41.64-31.94)/31.94
% NUBIA: (56.11-34.99)/34.99




% Table~\ref{tab:overall-study} presents average of METEOR, METEOR and NUBIA on all the patch description generated by \toolname{} and compared techiniques.
% As shown by the table, \toolname{} outperforms all the compared techniques including the base technique xx on all metrics significantly, indicating effectinessness in patch description generations.
% For example, the improvements achieved \toolname{} range from  x to XX, x to XX, and x to X in METEOR, BLEURT and NUBIA, respectively.

\noindent\textbf{Case analysis.} We further perform case analysis to illustrate the differences between \toolname{} and existing patch description generation methods. For instance, Figure~\ref{fig:eval-compared-example} showcases a case that includes patch code, the developer's original description (ground truth), and the descriptions generated by \toolname{} and other compared techniques.
In this case, developers addressed a potential memory leak by adding \texttt{usb\_put\_dev()} to the code. 
While the ground truth, which written by developers, describes the vulnerability and the fixing operation clearly, methods like RACE, RACE$_{history}$, CodeT5, and CodeReviewer typically generate brief summaries  Specifically, RACE, RACE$_{history}$, and CodeT5 merely mention that a memory leak was fixed, while CodeReviewer superficially describes the patch's operation. They both fail to detail the underlying reasons for the patch.
In contrast, \toolname{} generates more clear descriptions.
It accurately explains that the memory leak is caused by improper reference management and the fixing behavior: \textit{``... not properly release the USB device reference...''}.
% which is closely align with the ground truth.
% It harnesses the LLMs' capabilities in both code understanding and natural language generation to understand and describe patch.
By providing fluent, clear explanations of the patch's behavior and underlying rationale, \toolname{} aligns closely with the ground truth and outperforms other methods across all three metrics. 
The results highlight its superior capabilities in generating informative, accurate patch descriptions. Note that we use high-quality ground truth to evaluate generated description quality, aiming for ease of understanding and accurate evaluations. Yet, it's worth mentioning that a significant portion of real-world descriptions lack the details necessary for a comprehensive understanding of patches. We discuss this in the next section.

% \add{This tendency to produce similar, succinct summaries is reflected in the close scores these methods received across three key dimensions. They generally offer what might be considered just a part of a comprehensive patch description, focusing more on brevity than depth.}

% \add{
% In contrast, \toolname{} stands out for its ability to generate well-written security patch descriptions. Leveraging LLMs' capabilities for text generation and code understanding, \toolname{} comprehensively interprets the security patch. This approach brings \toolname{}'s output much closer to the ground truth, resulting in higher scores across all evaluated dimensions. By providing a more nuanced and complete description, \toolname{} demonstrates a significant advantage over other methods, highlighting its superior text generation and code understanding capabilities.}

% \textbf{case study.}
% The scores for the results of all four approaches are very similar, and they all generate results that are characterized as very short and are rather stiff, not fluent, and in some cases not even a readable sentence. These techniques are far away satisfactory for security patch generation.
% \todo{introduce the cases and summary}

\begin{figure}[ht]
\centering
% \vspace{-5px}
\includegraphics[width=1.0\linewidth]{images/compared_example.pdf}
\vspace{-10px}
\caption{Case analysis: generated descriptions across  methods }
\label{fig:eval-compared-example}
\vspace{5px}
\end{figure}
% \yuan{It is clear that our method is much better than the compared methods. However, grouth seems to be similiar to our method. Please highlight why our method is much better.}
% \subsubsection{Quality Distribution of Patch Description}

% \add{case study}
% % \add{Box plot}
% \add{Quality Distribution of Patch Description}
\vspace{-8px}
\subsection{Study of Real-World Descriptions}
To evaluate the real-world utility of \toolname{}, we evaluate the quality of existing patch descriptions in real-world, focusing on their comprehensiveness. Specifically, we select software repositories that each contains over 100 security patches in PatchDB. For each software repository, we randomly sample 100 security patches and evaluate their descriptions, using the comprehensiveness criteria described in Section~\ref{compared-with-sota}.
% comprehensiveness
The results are in displayed in Table~\ref{table:real-world-desc-quality}, indicate that the Linux Kernel has the highest quality of descriptions, with \todo{63\%} comprehensively detailing both \textit{what} and \textit{why} aspects. This finding also aligns with previous work~\cite{lin2023detecting}. Linux kernel community has a well-established patch management process and their patch descriptions typically offer detailed and explicit explanations. 
% Similarly, Qemu also exhibits good description quality with \todo{48\%} are comprehensive. 
However, some software, like php-src and radare2, displayed lower description quality. 
Their patches typically provided short descriptions, such as \textit{``Fix crash''}, lacking detailed explanations.
% On average, \todo{47.14\%} of the descriptions are comprehensive, leaving more than half of descriptions for improvement. 
While developers know their patches well, writing high-quality can be tedious, and developers often write short ones to finish faster. 
In contrast, as previously evaluated, \toolname{} demonstrates effectiveness in generating comprehensive and semantically accurate descriptions, showing its potential to improve the quality of security patch descriptions. 
We further introduce the case in Section~\ref{downstream_task}.

\ignore{
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Results of descriptions’ comprehensiveness across software}
\begin{tabular}{l|c|ccc}
\toprule
\textbf{Software}       & \cellcolor{gray!25}\textbf{All}  & \textbf{What} & \textbf{Why}  & \textbf{None} \\ \hline
Linux kernel   & \cellcolor{gray!25}84.00\% & 15.00\% & 0.00\%  & 1.00\%  \\ 
Qemu        & \cellcolor{gray!25}69.00\% & 29.00\% & 2.00\%  & 0.00\%  \\
FFmpeg      & \cellcolor{gray!25}47.00\% & 47.00\% & 3.00\%  & 3.00\%  \\ 
ImageMagick & \cellcolor{gray!25}39.00\% & 27.00\% & 0.00\%  & 31.00\% \\ 
php-src     & \cellcolor{gray!25}32.00\% & 63.00\% & 2.00\%  & 3.00\%  \\ 
wireshark   & \cellcolor{gray!25}30.00\% & 59.00\% & 9.00\%  & 2.00\%  \\ 
radare2     & \cellcolor{gray!25}29.00\% & 64.00\% & 0.00\%  & 7.00\%  \\ 
\bottomrule
\end{tabular}
\label{table:real-world-desc-quality}
\end{table}
}

\ignore{
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Results of descriptions’ comprehensiveness across software}
\begin{tabular}{l|c|ccc}
\toprule
\textbf{Software}       & \cellcolor{gray!25}\textbf{All}  & \textbf{What} & \textbf{Why}  & \textbf{None} \\ \hline
Linux kernel   & \cellcolor{gray!25}8.00\% & 73.00\% & 3.00\%  & 16.00\%  \\ 
php-src        & \cellcolor{gray!25}0.00\% & 10.00\% & 0.00\%  & 90.00\%  \\
radare2        & \cellcolor{gray!25}0.00\% & 6.00\% & 0.00\%  & 94.00\%  \\ 
FFmpeg         & \cellcolor{gray!25}4.00\% & 40.00\% & 0.00\%  & 56.00\%  \\ 
ImageMagick    & \cellcolor{gray!25}10.00\% & 8.00\% & 1.00\%  & 81.00\%  \\ 
qemu           & \cellcolor{gray!25}7.00\% & 62.00\% & 0.00\%  & 31.00\%  \\ 
wireshark      & \cellcolor{gray!25}1.00\% & 35.00\% & 0.00\%  & 64.00\%  \\ 
\bottomrule
\end{tabular}
\label{table:real-world-desc-quality}
\end{table}
}



\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\vspace{3px}
\caption{Results of descriptions’ comprehensiveness across software}
\begin{tabular}{l|c|ccc}
\toprule
\textbf{Software}       & \cellcolor{gray!25}\textbf{All}  & \textbf{What} & \textbf{Why}  & \textbf{None} \\ \hline
Linux                   & \cellcolor{gray!25}63\% & 31\% & 0\%  & 6\%  \\ 
Qemu                    & \cellcolor{gray!25}48\% & 50\% & 0\%  & 2\%  \\ 
ImageMagick             & \cellcolor{gray!25}23\% & 41\% & 0\%  & 36\%  \\ 
wireshark               & \cellcolor{gray!25}14\% & 71\% & 0\%  & 15\%  \\ 
FFmpeg                  & \cellcolor{gray!25}11\% & 84\% & 0\%  & 5\%  \\ 
php-src                 & \cellcolor{gray!25}2\% & 58\% & 2\%  & 38\%  \\
radare2                 & \cellcolor{gray!25}0\% & 73\% & 0\%  & 27\%  \\ 
\bottomrule
\end{tabular}
\label{table:real-world-desc-quality}
\end{table}


\ignore{
Besides, descriptions generated by \toolname{} can inevitably contain some errors compared to developer-written ones. It's important to note that developers are deeply familiar with their patches. And developer-written descriptions, collected from the open-source community, have undergone reviews among developers, reducing the likelihood of errors. In contrast, \toolname{} might produce inaccuracies due to model limitations. Automatically correcting these inaccuracies is highly challenging. Nevertheless, such inaccuracies usually make up only a small part of the overall descriptions. With minor adjustments, developers can easily refine these descriptions for use.}


\vspace{-8px}
\subsection{Impact Analysis on Downstream Task}
\label{downstream_task}
To further demonstrate \toolname{}'s utility, we evaluate its impact on downstream tasks.
Specifically, we selected APHP~\cite{lin2023detecting}, a tool that utilizes both patch code and descriptions to extract API usage specifications for bug detection.
In the evaluation, we collect 100 patches from APHP's list of patches, specifically those where APHP initially failed to extract specifications. We generated new descriptions for these patches using \toolname{} and reprocessed them with APHP. The results were promising, showing successful specification extraction in \todo{11\%} of cases using \toolname{}-generated descriptions. The evaluation shows that \toolname{} can improve the performance of downstream tasks that rely on the quality of patch descriptions.
% APHP primarily extracts critical elements such as the target API from patch descriptions. Original descriptions lacking in key details or omitting the target API often result in failed extractions, subsequently affecting bug detection. In contrast, \toolname{} can generated comprehensive descriptions that mention key details, thus enhancing APHP's extraction capability.
% For instance. Figure~\ref{fig:downstream-impact} displays a security patch from Qemu. The original developer's description, while mentioning the patch actions, missed essential details like the critical API for memory allocation, 
% hindering APHP from extracting API specifications. In contrast, the \toolname{}-generated description clearly highlighting the key API \texttt{g\_strdup\_printf} related to vulnerability. This facilitated APHP in successfully extracting the API specification. 
For instance. Figure~\ref{fig:downstream-impact} displays a security patch from Qemu. The original developer's description, while mentioning the patch actions, missed essential details like the critical API for memory allocation, which is essential for understanding the vulnerability's cause. 
% In contrast, the description generated by \toolname{} explicitly highlights the critical API \texttt{g\_strdup\_printf}, directly related to the vulnerability. This clarity significantly aided APHP in successfully extracting the API specification.
In contrast, the description generated by \toolname{} explicitly highlights the critical API \texttt{g\_strdup\_printf}, directly related to the vulnerability. This advantage stems from the context-aware diff generation, which augments the prompt with relevant context, despite the critical API call not being in the default patch code. This context facilitates LLMs in producing more useful descriptions and assisting APHP in successfully extracting the API specification.

% efficiently identifying, categorizing, and prioritizing patches based on the mentioned security impacts, leading to quicker responses to critical security issues. 
Besides, such comprehensive descriptions aid developers in patch propagation.
During propagation, security patches may not be directly applicable to different versions. Developers typically need to adjust them to fix vulnerabilities, including changing the patch position, fitting the code context, and modifying the fix logic~\cite{tan2022understanding}. In this process, descriptions can facilitate a better understanding of the vulnerability, enabling appropriate adjustments. For example, the description indicates that the vulnerability is related to the API \textit{``g\_strdup\_printf''} call. With this understanding, developers can locate the call to this API and adjust the code changes accordingly, enabling swift deployment.


% In addition, during the patch propagation, comprehensive descriptions guide developers in adapting patches to various contexts. For example, the description indicates that the vulnerability is related to the API \textit{``g\_strdup\_printf''} call. With this understanding, developers can locate the call to this API and adjust the code changes accordingly, enabling swift deployment.

% detailing the vulnerabilities and fixing operations 
\begin{figure}[ht]
\centering
% \vspace{-13px}
\includegraphics[width=0.9\linewidth]{images/case-for-downstream.pdf}
\vspace{-8px}
\caption{Case analysis: developer-written and \toolname{}'s description}
\label{fig:downstream-impact}
\vspace{-8px}
\end{figure}



\ignore{
\subsection{Ablation Study}
% \noindent\textbf{Comparison method.} 
% To assess the impact of \toolname{}'s design, we conducted a modular evaluation. Specifically, To evaluate the effectiveness of the designed instruction, patch-code specific prompts, and the inconsistency-checking mechanism. As we know, when using LLMs, prompt is very important and has a lot to do with the quality of the output.
% As we have described, our prompt is divided into two parts, the instruction and the patch code, which is different for each patch. 
% Since these two parts of the design have different strategies and are relatively independent of each other, we evaluate the effectiveness of these two pieces of the design separately.
% We designed the following variants of \toolname{} and comparing descriptions generated by them:
To evaluate the individual impact of various components within \toolname{}, we perform a modular evaluation. Our prompt comprises two primary elements: the instruction and the patch code. Given their distinct strategies and relative independence, we examined the effectiveness of them separately.
Therefore, we use the following \toolname{} variants to evaluate three components: the designed instruction, patch-code specific prompts, and the inconsistency-checking mechanism. 


% as shown in Figure~\ref{fig:llm-baisc-prompt}
% \vspace{2pt}\noindent$\bullet$ \textbf{LLM-basic:} We start with the most basic system, LLM-base, which uses a straightforward prompt design: \textit{``Write a commit message for the following patch code:
% {{patch code}}.''} It utilizes LLMs with direct instruction, composed with code changes as code input and uses straightforward LLMs outputs. This prototype serves as our baseline to provide a direct comparison for further enhancements.

\vspace{2pt}\noindent$\bullet$ \textbf{LLM-basic:} As our baseline, LLM-basic employs a simple prompt template: \textit{``Write a commit message for the following patch code: {\{patch code\}}.''} This variant uses basic LLMs directly with straightforward prompt instruction and code changes in patches. 
% It provides a baseline for subsequent enhancements.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=1.0\linewidth]{images/tool-basic-prompt-instruction-testing.pdf}
% \caption{Prompt design for LLM-basic}
% \label{fig:llm-baisc-prompt}
% \end{figure}

% \vspace{2pt}\noindent$\bullet$ \textbf{\toolname{}$_{instr}$:} To assess the impact of custom instructions on the results, we modify LLM-basic by replacing its instruction with the designed instruction while keeping other aspects unchanged. This variant helps us understand the value added by tailored instructions.
\vspace{2pt}\noindent$\bullet$ \textbf{\toolname{}$_{instr}$:} This variant, an evolution of LLM-basic, replace its instruction with the designed instruction (shown in Figure~\ref{fig:prompt-design}) to understand its impact on the generated output while keeping other components constant.


% \vspace{2pt}\noindent$\bullet$ \textbf{\toolname{}$_{code}$}: Building on \toolname{}$_{instr}$, this variants incorporates patch-code specific prompts to evaluate its influence on the results. Here, the patch code's changes in \toolname{}$_{instr}$ are replaced with results obtained from our patch-code slicing technique.

\vspace{2pt}\noindent$\bullet$ \textbf{\toolname{}$_{code}$:} Building further, \toolname{}$_{code}$ integrates patch-code specific prompts. Here, the code changes in \toolname{}$_{instr}$ are replaced with results obtained from our patch-code slicing technique.

% \vspace{2pt}\noindent$\bullet$ \textbf{\toolname{}$_{check}$}: To evaluate the effectiveness of the inconsistency checker, we enhance \toolname{}$_{code}$ by integrating the checker and filtering out reported inconsistencies. 
\vspace{2pt}\noindent$\bullet$ \textbf{\toolname{}$_{check}$:} The final variant, \toolname{}$_{check}$, extends \toolname{}$_{code}$ by incorporating an inconsistency checker to refine the output by identifying and filtering out inconsistencies. 


% By incrementally building these prototypes, we can assess the contributions of individual components of \toolname{}. Table~\ref{tab:ablation-study} details the effectiveness of each variant. 
In the following sections, we then analyze the contribution of each component quantitatively and qualitatively.


 
% \subsubsection{Contribution of instruction in prompt}
\ignore{
\begin{table}[ht]
\caption{Results of the ablation study}
\centering
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|ccc}
\toprule
\textbf{Model} & \textbf{METEOR} & \textbf{BLEURT} & \textbf{NUBIA} \\
\toprule
LLM-basic           & 11.62           & 38.1         & 44.03         \\

\toolname{}$_{instr}$  & 16.36            & 41.04           & 53.43          \\

\toolname{}$_{code}$         & 17.11           & 41.64         & 56.11          \\

\toolname{}$_{check}$   & -               & -               & -              \\
% \hline
% SecDescribler  & \textbf{16.99}           & \textbf{41.65}           & \textbf{55.1}  \\   
\bottomrule  
\end{tabular}
\label{tab:ablation-study}
\end{table}
}


% \begin{figure}[ht]
% \centering
% \includegraphics[width=1.0\linewidth]{images/mo}
% \caption{Prompt design for LLM-basic}
% \label{fig:llm-baisc-prompt}
% \end{figure}

\ignore{
\begin{table}[]
\begin{tabular}{cccc}
\textbf{Prompt} & \textbf{METEOR} & \textbf{BLEURT} & \textbf{NUBIA} \\
Basic Prompt    & 11.62           & 38.1            & 44.03          \\
Enhanced Prompt & 16.99           & 41.65           & 55.1           \\
\end{tabular}
\end{table}

% \subsubsection{Contribution of code in prompt}

\begin{table}[]
\begin{tabular}{cccc}
\textbf{Model}            & \textbf{METEOR}               & \textbf{BLEURT}    & \textbf{NUBIA}               \\
SecDescribler w/o checker & 16.99 &41.65 & 55.1 \\
SecDescribler             & -                             & -                  & -  
\end{tabular}
\end{table}

\begin{table}[]
\begin{tabular}{cccc}
\textbf{Patch code}     & \textbf{METEOR}               & \textbf{BLEURT}               & \textbf{NUBIA}                \\
code changes            & 16.36 & 41.04 & 53.43 \\
code changes w/ slicing & 16.99 & 41.65 & 55.1 \\
\end{tabular}
\end{table}
}


\ignore{
\subsubsection{Effectiveness of the designed instruction.}
As shown in Table~\ref{tab:ablation-study}, the effectiveness of \toolname{}$_{instr}$ is better than LLMs-basic in terms of all three metrics,  
For example, the improvements achieved \toolname{} \todo{XX}\%, \todo{XX}\%, and \todo{XX}\%in METEOR, BLEURT and NUBIA, compared to LLM-basic, respectively. 
This indicates that including instruction helpful for effective patch description generation. 
% We further look into some cases that \toolname{}$_{instr}$ exhibits more effective than the LLMs-basic in terms of these metrics. Figure X presents such a real-world case, which includes the patch code, the ground truth, the patch descriptions generated by the \toolname{}$_{code}$, \toolname{}$_{instr}$. In this example, developers ...
% \add{case analysis}
After manually reviewing the generated results, we noticed distinct differences in style between LLM-basic and \toolname{}$_{instr}$. For example, for the patch shown in Figure~\ref{fig:eval-compared-example}, LLM-basic generates the description: \textit{``Add USB device release in error case to prevent memory leak.''} This description, while generally correct, lacks detailed explanation. LLM-basic's instructions are basic and straightforward, focusing solely on the task without additional guidance. This often leads LLMs to create brief, one-liner summaries. They frequently miss the depth and comprehensive insight necessary for a well-written security patch description. On the other hand, \toolname{}'s instructions provide a broader content framework, offering better guidance to LLMs. This enables the generation of descriptions that are both concise and informative.

These results show the impact of instruction design on the patch description generation capabilities of LLMs. While LLMs can produce smooth and coherent text, the quality of their output also heavily depend on the given instruction. Effective instruction stimulates the LLM's potential by providing clear direction. Conversely, a vague or overly broad instruction may result in the underutilization of the LLM's capabilities, yielding generic or superficial descriptions. 
}

 % enhancing the quality of the security patch descriptions
\ignore{
From the results, we can see that LLMs are sensitive to prompt instruction.
This instruction of LLM-basic is the basic and straightforward, defining the task without additional content guidance. In this way, this relies on LLMs inherent understanding of commit messages to generations. This led to led the LLM to generate brief, one-liner summaries. While these were succinct, they often lacked the depth and comprehensive insight needed for a well-written security patch description. In contrast, the instruction of \toolname{} provides a general content framework, better guide LLMs. It enabled the LLM to generate descriptions that were both concise and informative.
The results highlight the text generation capabilities of LLMs and their sensitivity to prompts. LLMs can produce smooth and coherent text, but their output is heavily influenced by the given prompt. In order to better stimulate the potential of large models, we should design appropriate prompts.
A vague or overly broad prompt can lead to underutilization of the LLM's potential, yielding generic or insufficiently detailed outputs.
}


\subsubsection{Effectiveness of context-aware diff generation.}

% As shown in Table~\ref{tab:ablation-study}, the effectiveness of \toolname{}$_{code}$ is better than \toolname{}$_{instr}$ in terms of all three metrics, indicating that including patch-specific prompt construction helpful for patch description generation.
\ignore{
As shown in Table~\ref{tab:ablation-study}, the effectiveness of \toolname{}$_{code}$ is better than \toolname{}$_{instr}$ in terms of all three metrics,  
Specifically, the improvements achieved \toolname{}$_{code}$ \todo{XX}\%, \todo{XX}\%, and \todo{XX}\%in METEOR, BLEURT and NUBIA, compared to \toolname{}$_{instr}$, respectively. 
\toolname{} improves input quality by incorporating patch context. In this way, LLMs not only enrich descriptions but also enhance their understanding of patches, thus producing better descriptions.
}

\ignore{
As shown in Table~\ref{tab:ablation-study}, the effectiveness of \toolname{}$_{code}$ is better than \toolname{}$_{instr}$ in terms of all three metrics: METEOR, BLEURT, and NUBIA. Specifically, \toolname{}${code}$ shows improvements of \todo{XX\%}, \todo{XX\%}, and \todo{XX\%} in each metric respectively compared to \toolname{}${instr}$. 
These results show the advantage of incorporating patch context into input quality. By doing so, LLMs not only produce more enriched descriptions but also gain a better understanding of the patches, leading to better descriptions. 
We further look into cases that \toolname{}$_{code}$ exhibits more effective than the \toolname{}$_{instr}$ in terms of these metrics. We find that \toolname{}$_{code}$ generates descriptions that more accurately reflect the underlying reasons behind the patch, such as the nature of the vulnerability and its security impacts. In contrast, \toolname{}$_{instr}$ provides direct code changes, which is directly related to what the patch does,  thus already enabling LLMs to the patch's actions.  And the additional context provided by \toolname{}$_{code}$ allows LLMs to capture the reasons behind these changes, thus facilitating the description generation.
}

As shown in Table~\ref{tab:ablation-study}, the effectiveness of \toolname{}$_{code}$ is better than \toolname{}$_{instr}$ in terms of all three metrics: METEOR, BLEURT, and NUBIA. Specifically, \toolname{}${code}$ shows improvements of \todo{XX\%}, \todo{XX\%}, and \todo{XX\%} in each metric respectively compared to \toolname{}${instr}$.
We further look into cases that \toolname{}$_{code}$ exhibits more effective than the \toolname{}$_{instr}$. We find that \toolname{}$_{code}$ is better at capturing the underlying reasons behind patches, such as the vulnerability and its security impacts. In contrast, \toolname{}$_{instr}$ provides direct code changes, and thus primarily describes the patch's operations. These results show the benefits of incorporating patch context into prompts. By doing so, LLMs gain a better understanding of the patches, leading to more informative descriptions. For example, with the extracted context, the LLMs generate a more detailed description for patch in Figure~\ref{fig:desc-kzalloc-CVE-2019-19536}, as depicted in Figure ~\ref{fig:desc-with-context}. This description mentions that \textit{``the function didn't check if the kmalloc function ... If kmalloc failed to allocate memory ...''}. Compared to the description of the generation with only code changes in Figure~\ref{fig:desc-lacking-context} (b), this description describes more specifically the vulnerability cause, thus helping other developers better understand the patch code.


\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{images/tool-case-for-prompt-generation-3.pdf}
\caption{\toolname{}'s description for CVE-2022-3106}
\label{fig:desc-with-context}
\end{figure}
% with necessary context


% We further look into some cases that \toolname{}$_{code}$ exhibits more effective than the \toolname{}$_{instr}$ in terms of these metrics. Figure X presents such a real-world case, which includes the patch code, the ground truth, the patch descriptions generated by the default \toolname{}$_{code}$, \toolname{}$_{instr}$, and other compared techniques. In this example, developers ...
% ...
% In particular, comparing \toolname{}-- with LLM-basic, we can see the patch-specific prompt construction module helps to increase the percentages of describing all three metrics. 
% For the \textit{All} aspect, it increases the percentage of by \todo{15\%} under the GPT-3.5 model, and \todo{9\%} under the GPT-4 model, respectively. 

% Besides, \toolname{} displays more improvement in describing \textit{vulnerability causes} and \textit{security impacts}, compared to \textit{fixing operation}. LLM-basic provides code change information, which is directly related to \textit{fixing operation}, thus already enabling the LLMs to describe it directly. As contexts provide additional information about the vulnerability cause and the potential security impact, \toolname{}’s primary advancements are concentrated on the description of \textit{vulnerability cause} and \textit{security impact}.


% \add{case analysis: for patch-specific prompt construction.+ designed instruction.}


\subsubsection{Effectiveness of code-description inconsistency checking.}
As shown in Table~\ref{tab:ablation-study}, the effectiveness of \toolname{}$_{code}$ is better than \toolname{}$_{instr}$ in terms of all three metrics: METEOR, BLEURT, and NUBIA. Specifically, \toolname{}${code}$ shows improvements of \todo{XX\%}, \todo{XX\%}, and \todo{XX\%} in each metric respectively compared to \toolname{}${instr}$. 
% Under the GPT-3.5 model, the percentage of \textit{All} increased by \todo{6\%}, and under the GPT-4 model, it increased by \todo{21\%}. 
LLMs output is not only dependent on the quality of input data. It is also significantly influenced by LLMs' inherent capabilities. Therefore, with code-description inconsistency checking, \toolname{} can further improve the effectiveness using LLMs.

% \add{case analysis:}


\ignore{
We analyze the cases where \toolname{} fails to correctly describe security-related details. These errors are not recognized by \toolname{} for three main reasons.
\ding{182} First, the unstructured nature of the text may hinder effective key-detail extraction thus preventing subsequent verification. 
For instance, \toolname{} overlooks the wrong fixing action \textit{``checks''} from the statement \textit{``The patches fix this by adding additional checks''} even though the code does not introduce new checks. 
\ding{183} Second, the vulnerability type and the corresponding fixing statement type are not one-to-one. Multiple vulnerability types may share the same statement type. For example, both memory leak and buffer overflow vulnerabilities might relate to call statements in patches. Thus, when a memory leak is misdescribed as a buffer overflow, \toolname{} cannot detect the inconsistency due to this overlap. \ding{184} Third, the description may contain errors about other types of information, such as the vulnerability trigger conditions, which are uncovered by \toolname{} currently. 
}


\ignore{
Besides, descriptions generated by \toolname{} can inevitably contain some errors compared to human-written ones. It's important to note that developers are deeply familiar with their patches. And human-written descriptions, collected from the open-source community, have undergone reviews among developers, reducing the likelihood of errors. In contrast, \toolname{} might produce inaccuracies due to model limitations. Automatically correcting these inaccuracies is highly challenging. Nevertheless, such inaccuracies usually make up only a small part of the overall descriptions. With minor adjustments, developers can easily refine these descriptions for use.
}

From the evaluation, we can see that three parts all enhance the generation of security patch descriptions:
Firstly, accurate instructions are vital. They guide LLMs to produce relevant and precise content. Well-crafted instruction ensures the LLMs' outputs closely align with the specific requirements of the patch description.
Secondly, providing the LLMs with proper context is essential for understanding and accurately describing patches. 
Lastly, due to the probabilistic nature of LLMs, variation in quality is inevitable, regardless of how refined the prompts are. Inconsistency checking comes to mitigates the inherent uncertainties in model outputs, enhancing their reliability.
Each part plays a crucial role, and while their individual contributions vary, they collectively improve the model's performance. By combining the three parts, \toolname{} effectively leverages the strengths of LLMs to generate more accurate and reliable security patch descriptions.
}


\ignore{
From the evaluation, we can see that three key factors critically enhance the generation of security patch descriptions, Each element plays an indispensable role, and while their individual enhacement varies, they collectively enhance the model's performance:
First, accurate instructions are crucial. They direct (LLMs) to produce relevant and precise content. Well-crafted prompts ensure the LLMs' outputs align closely with the specific requirements of the patch description. 
Besides, LLMs need the proper context to understand and describe patches accurately. Even with powerful LLMs, the absence of sufficient context regarding the current patch and its associated vulnerabilities hampers the model's ability to comprehend and accurately describe the patch. It's crucial to provide relevant contextual information that the model cannot infer from its training alone. 
In addition, given the probabilistic nature of LLMs, no matter how much we refine the prompts, the results can vary in quality. Therefore, employing external tools to check the LLM's output is vital. This step helps quickly identify and rectify any issues, ensuring the final descriptions are of high quality. Inconsistency checking of results mitigates the inherent uncertainties in model outputs, enhancing reliability.
These aspects independently contributes to improving the results. They are not interchangeable and have their unique areas of impact. By combining precise instructions, relevant contextual information, and rigorous result checking, \toolname{} effectively leveraging the strengths of LLMs to generate more accurate and reliable security patch descriptions. 
}
